Improving Knowledge Distillation via Regularizing Feature Norm and Direction

Knowledge distillation (KD) exploits a large well-trained model (i.e., teacher) to train a small student model on the same dataset for the same task. Treating teacher features as knowledge, prevailing methods of knowledge distillation train student by aligning its features with the teacher's, e.g., by minimizing the KL-divergence between their logits or L2 distance between their intermediate features. While it is natural to believe that better alignment of student features to the teacher better distills teacher knowledge, simply forcing this alignment does not directly contribute to the student's performance, e.g., classification accuracy. In this work, we propose to align student features with class-mean of teacher features, where class-mean naturally serves as a strong classifier. To this end, we explore baseline techniques such as adopting the cosine distance based loss to encourage the similarity between student features and their corresponding class-means of the teacher. Moreover, we train the student to produce large-norm features, inspired by other lines of work (e.g., model pruning and domain adaptation), which find the large-norm features to be more significant. Finally, we propose a rather simple loss term (dubbed ND loss) to simultaneously (1) encourage student to produce large-\emph{norm} features, and (2) align the \emph{direction} of student features and teacher class-means. Experiments on standard benchmarks demonstrate that our explored techniques help existing KD methods achieve better performance, i.e., higher classification accuracy on ImageNet and CIFAR100 datasets, and higher detection precision on COCO dataset. Importantly, our proposed ND loss helps the most, leading to the state-of-the-art performance on these benchmarks. The source code is available at \url{https://github.com/WangYZ1608/Knowledge-Distillation-via-ND}.

==> figures/larger_teacher.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width = 0.32\textwidth]{images/acckd.pdf}
    \includegraphics[width = 0.32\textwidth]{images/accdkd.pdf}
    \includegraphics[width = 0.32\textwidth]{images/accrkd.pdf}

\vspace{2.5mm}
\caption{\textbf{Our method can benefit from larger teachers.} With the teacher capacity increasing, our method, KD++, DKD++ and ReviewKD++ (\textcolor{red}{\textbf{red}}) is able to learn better distillation results, even though the original distillation frameworks (\textcolor{blue}{\textbf{blue}}) suffers from degradation problems. The student is ResNet-18, teacher is changed from ResNet-34 to ResNet-152, and reported the Top-1 accuracy ($\%$) on the ImageNet validation set.}
\label{fig:larger_tea}
\end{figure}

==> tables/Ablation.tex <==
\begin{table}
    \begin{subtable}[h]{0.30\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        % CE  & 64.60\\
        CE+KL(\textit{baseline}) & 67.65\\
        CE+ND & 68.78\\
        ND+KL & 68.68\\
        CE+ND+KL & \colorbox{lightgray}{\textbf{70.10}}\\
       \end{tabular}
       \vspace{1.0mm}
       \caption{\textbf{larger norm and consist direction}. ND is good for knowledge transfer.}\label{EFA}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.40\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lcc}
        case & R50$\rightarrow$MV2 & R56$\rightarrow $R20\\
        \hline
        \toprule
        \textit{baseline} & 67.65 & 70.66\\
        % \hline
        % \textit{only direction} & ~ & ~\\
        cosine & 69.18 & 71.75\\
        InfoNCE   & 69.06 & 70.73\\
        &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{only direction}. Constraining only the features direction can also improve accuracy. \textit{cosine} is suitable for more diverse nets.}\label{direction}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.25\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        % \textit{only norm} & ~\\
        \textit{baseline} & 67.65\\
        MSE & 69.05\\
        SFN & 69.32\\
         &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{only norm}. Constraining only the features norm can also improve accuracy.}\label{norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.30\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        cosine w/ MSE & 68.62\\
        cosine w/ SFN & 69.07\\
        InfoNCE w/ MSE & 68.47\\
        InfoNCE w/ SFN & 68.71\\
        ND           & \colorbox{lightgray}{\textbf{70.10}}\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{direction w/ norm}. ND take advantage of both direction and norm.}\label{dir-norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.41\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{ccc}
        \textit{k} & R50$\rightarrow$MV2 & R56$\rightarrow $R20\\
        \hline
        \toprule
        -0.5 & 69.46 & 71.57\\
        0.0    & \colorbox{lightgray}{\textbf{70.10}} & \colorbox{lightgray}{\textbf{72.53}}\\
        0.5	 & 70.23	& 71.86\\
        1.0	 & 69.72	& 71.79\\
        1.5	 & 68.49	& 71.74\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{scale teacher norm}. Norm is sensitive to \textit{k}, and it is sufficient to use the teacher norm as the learning objective.\shu{where is $k$ used, what equations?}}
        \label{tea-norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.25\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        % \textit{only norm} & ~\\
        easy samples & 72.01\\
        all samples  & \colorbox{lightgray}{\textbf{71.98}}\\
         &\\
         &\\
         &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{sample strategy}. Sampling strategy has little effect on distillation.}\label{sample}
    \end{subtable}
\vspace{2.5mm}
\caption{\textbf{Ablation experiments on CIFAR-100.} We report accuracy on the test set. If not specified, the default is: the teacher and student are ResNet-50 and MobileNet-V2, respectively, and student trained by Eq.~\ref{eq8}. We count the mean of the teacher's embedding features for each category on the whole training set as the category center. Default settings are marked in \colorbox{lightgray}{gray}.}
\label{tab:ablation}
\end{table}

==> tables/ImageNet-ViT.tex <==
\begin{table}[h]
    \centering
        \renewcommand{\arraystretch}{1.2}
        % \setlength\tabcolsep{3.5pt}
        \resizebox{0.75\textwidth}{!}{%
        % \small
        \begin{tabular}{cccc|cc|cc}
        Student & Teacher & Student & Teacher & KD\cite{hinton2015distilling} & DKD$^{*}$\cite{zhao2022decoupled} & \textbf{KD++} & \textbf{DKD++}\\
        \hline
        \toprule
        \multirow{2}{*}{ResNet-18} & ViT-S & \multirow{2}{*}{69.76} & 74.64 & ~ & ~ & ~ & ~\\
        ~ & ViT-B & ~ & 78.00 & ~ & ~ & ~ & ~\\
        \end{tabular}
    }
    \vspace{2.5mm}
    \caption{vit distilled to cnn.}
    \label{tab:imagenet-vit}
\end{table}

==> tables/suppl_ablation.tex <==
\begin{table}
    \begin{subtable}[h]{0.28\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        \textit{baseline} & 67.65\\
        MSE & 69.05\\
        SIFN & 69.32\\
        &\\
        &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{Regularizing feature \textbf{norm} only improve accuracy.}\label{norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.38\textwidth}
        \setlength\tabcolsep{1.5pt}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lcc}
        case & R50$\rightarrow$MV2 & R56$\rightarrow $R20\\
        \hline
        \toprule
        \textit{baseline} & 67.65 & 70.66\\
        % \hline
        % \textit{only direction} & ~ & ~\\
        cosine & 69.18 & 71.75\\
        InfoNCE   & 69.06 & 70.73\\
        &\\
        &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{Regularizing feature \textbf{direction} only. \textit{Cosine} is suitable for more diverse nets.}\label{direction}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.30\textwidth}
        \setlength\tabcolsep{1.5pt}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        cosine w/ MSE & 68.62\\
        cosine w/ SIFN & 69.07\\
        InfoNCE w/ MSE & 68.47\\
        InfoNCE w/ SIFN & 68.71\\
        ND           & \colorbox{lightgray}{\textbf{70.10}}\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{Regularizing \textbf{direction w/ norm}. ND works the best.}\label{dir-norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.35\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{ccc}
        \textit{k} & R50$\rightarrow$MV2 & R56$\rightarrow $R20\\
        \hline
        \toprule
        -0.5 & 69.46 & 71.57\\
        0.0    & \colorbox{lightgray}{\textbf{70.10}} & \colorbox{lightgray}{\textbf{72.53}}\\
        0.5	 & 70.23	& 71.86\\
        1.0	 & 69.72	& 71.79\\
        1.5	 & 68.49	& 71.74\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{scale teacher norm}. use the teacher norm as the learning objective.}
        \label{tea-norm}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.25\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{lc}
        case &  acc.\\
        \hline
        \toprule
        % \textit{only norm} & ~\\
        easy samples & 72.01\\
        all samples  & \colorbox{lightgray}{\textbf{71.98}}\\
         &\\
         &\\
         &\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{\textbf{sample strategy} has little effect on distillation.}\label{sample}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.18\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{cc}
        $\beta$ &  acc.\\
        \hline
        \toprule
        0.5  & 69.37\\
        1.0  & 68.64\\
        2.0  & 69.19\\
        3.0  & 67.32\\
        4.0  & 68.58\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{Sensitivity of \textbf{$\beta$}. $(\alpha=1.0)$.}\label{beta}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.18\textwidth}
        \renewcommand{\arraystretch}{1.2}
        \small
        \centering
        \begin{tabular}{cc}
        $\alpha$ &  acc.\\
        \hline
        \toprule
        0.5  & 68.61\\
        1.0  & 68.69\\
        2.0  & 69.07\\
        3.0  & \colorbox{lightgray}{\textbf{70.10}}\\
        4.0  & 69.83\\
        \end{tabular}
        \vspace{1.5mm}
        \caption{ Sensitivity of \textbf{$\alpha$}. $(\beta=0.5)$.}\label{alpha}
    \end{subtable}
\vspace{2.5mm}
\caption{\textbf{Ablation experiments on CIFAR-100.} We report accuracy on the test set. If not specified, the default is: the teacher and student are ResNet-50 and MobileNet-V2, respectively, and student trained by Eq.8. We count the mean of the teacher's embedding features for each category on the whole training set as the category center. Default settings are marked in \colorbox{lightgray}{gray}.}
\label{tab:suppl_ablation}
\end{table}

==> tables/suppl_dir_norm.tex <==
% \begin{table}[h]
%     \centering
%     \caption{
%     }
%     \vspace{1mm}
%         \renewcommand{\arraystretch}{1.2}
%         % \setlength\tabcolsep{1.5pt}
%         \resizebox{0.9\textwidth}{!}{%
%         % \small
%         \begin{tabular}{c|c|cc|cc|ccccc}
%         \hline
%         methods & KD & \multicolumn{2}{c}{only Norm} & \multicolumn{2}{|c}{only Direction} & \multicolumn{5}{|c}{Direction w/ Norm}\\
%         \cline{2-11}
%         \hline
%         \textit{baseline} & $\checkmark$ & ~ & ~ & ~ & ~\\
%         \hline
%         MSE               & ~ & $\checkmark$ & ~ & ~ & ~ & $\checkmark$ & ~ & $\checkmark$\\
%         SIFN              & ~ & ~ & $\checkmark$ & ~ & ~ & ~ & $\checkmark$ & ~ & $\checkmark$\\
%         \hline
%         cosine            & ~ & ~ & ~ & $\checkmark$ & ~ & $\checkmark$ & $\checkmark$\\
%         InfoNCE           & ~ & ~ & ~ & ~ & $\checkmark$ & ~ & ~ & $\checkmark$ & $\checkmark$\\
%         \hline
%         \textbf{ND}                & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & $\checkmark$\\
%         \hline
%         Acc (\%) & 67.65 & 69.05 & 69.32 & 69.18 & 69.06 & 68.62 & 69.07 & 68.47 & 68.71 & \textbf{70.10}\\
%         \hline
%         \end{tabular}
%     }
%        %\vspace{1.5mm}
%         \label{tab:suppl_dir_norm}
% \end{table}

\begin{table}[h]
\centering
    \caption{}
    \vspace{1mm}
        \renewcommand{\arraystretch}{1.2}
        % \setlength\tabcolsep{1.5pt}
        \resizebox{0.7\textwidth}{!}{%
        % \small
        \begin{tabular}{ccccccc}
        \hline
        \textit{baseline} & \multicolumn{2}{c}{Regular Norm} & \multicolumn{2}{c}{Regular Direction} & ours & ~\\
        KD & MSE & SIFN & cosine & InfoNCE & \textbf{ND} & Acc (\%)\\
        \hline
        $\checkmark$ & ~ & ~ & ~ & ~ & ~ & 67.65\\
        ~ & $\checkmark$ & ~ & ~ & ~ & ~ & 69.05\\
        ~ & ~ & $\checkmark$ & ~ & ~ & ~ & 69.32\\
        ~ & ~ & ~ & $\checkmark$ & ~ & ~ & 69.18\\
        ~ & ~ & ~ & ~ & $\checkmark$ & ~ & 69.06\\
        ~ & $\checkmark$ & ~ & $\checkmark$ & ~ & ~ & 69.06\\
        ~ & ~ & $\checkmark$ & $\checkmark$ & ~ & ~ & 69.06\\
        ~ & $\checkmark$ & ~ & ~ & $\checkmark$ & ~ & 69.06\\
        ~ & ~ & $\checkmark$ & ~ & $\checkmark$ & ~ & 69.06\\
        ~ & ~ & ~ & ~ & ~ & $\checkmark$ & \textbf{70.10}\\
        \hline
        \end{tabular}
    }
    \label{tab:suppl_dir_norm}
\end{table}
